Measuring Tidal Dissipation in Giant Planets from Tidal Circularization

In this project, we determined the constraints on the modified tidal quality factor, $Q_{pl}'$, of gas-giant planets orbiting close to their host stars. We allowed $Q_{pl}'$ to depend on tidal frequency, accounting for the multiple tidal waves with time-dependent frequencies simultaneously present on the planet. We performed our analysis on 78 single-star and single-planet systems, with giant planets and host stars with radiative cores and convective outer shells. We extracted constraints on the frequency-dependent $Q_{pl}'$ for each system separately and combined them to find general constraints on $Q_{pl}'$ required to explain the observed eccentricity envelope while simultaneously allowing the observed eccentricities of all systems to survive to the present day. Individual systems do not place tight constraints on $Q_{pl}'$. However, since similar planets must have similar tidal dissipation, we require that a consistent, possibly frequency-dependent, model must apply. Under that assumption, we find that the value of $\log_{10}Q_{pl}'$ for HJs is $5.0\pm0.5$ for the range of tidal period from 0.8 to 7 days. We did not see any clear sign of frequency dependence of $Q_{pl}'$.

==> Acknowledgement.tex <==
\section*{Acknowledgements}

This research was supported by NASA grant 80NSSC18K1009. The authors acknowledge
the Texas Advanced Computing Center (TACC) at The University of Texas at Austin
for providing HPC resources that have contributed to the research results
reported in this article. URL: \url{http://www.tacc.utexas.edu}. The authors
would like to thank Dr. Adrian Barker for providing constructive and detailed
feedback which significantly improved this manuscript.



==> comp1.tex <==
\begin{tabular}{lcccccccccccc}
&&\multicolumn{5}{c@{}}{\textbf{Individual Quantiles of $\log_{10}Q'_{p}$}} & \multicolumn{5}{c}{\textbf{Combined Quantiles of $\log_{10}Q'_{p}$}}\\
\multicolumn{1}{l@{}}{\textbf{System}} & \multicolumn{1}{l@{}}{$P_{tide}$} & \multicolumn{1}{l@{}}{\textbf{2.3 \%}} & \multicolumn{1}{l@{}}{\textbf{15.9\%}} & \multicolumn{1}{l@{}}{\textbf{50.0\%}} & \multicolumn{1}{l@{}}{\textbf{84.1\%}} & \multicolumn{1}{l@{}}{\textbf{97.7\%}} & \multicolumn{1}{l@{}}{\textbf{2.3 \%}} & \multicolumn{1}{l@{}}{\textbf{15.9\%}} & \multicolumn{1}{l@{}}{\textbf{50.0\%}} & \multicolumn{1}{l@{}}{\textbf{84.1\%}} & \multicolumn{1}{l@{}}{\textbf{97.7\%}} \\
\hline
HATS-54 b & 0.50 & 3.33 & 4.02 & 5.36 & 7.00 & 11.61 & 5.60 & 5.93 & 6.23 & 6.90 & 8.14 \\
WASP-32 b & 0.76 & 3.08 & 3.50 & 4.48 & 5.73 & 9.99 & 4.76 & 5.02 & 5.65 & 5.83 & 6.20 \\
TOI-564 b & 0.84 & 3.12 & 3.82 & 5.25 & 7.20 & 9.89 & 4.75 & 4.89 & 5.40 & 5.82 & 6.28 \\
CoRoT-27 b & 1.14 & 3.10 & 3.56 & 4.46 & 6.48 & 10.47 & 4.64 & 4.75 & 4.94 & 5.12 & 5.24 \\
HAT-P-36 b & 1.27 & 3.19 & 4.02 & 5.61 & 7.16 & 7.84 & 4.59 & 4.70 & 4.88 & 5.05 & 5.19 \\
HATS-18 b & 1.27 & 3.10 & 3.92 & 5.79 & 7.32 & 8.24 & 4.59 & 4.70 & 4.88 & 5.05 & 5.19 \\
WASP-43 b & 1.27 & 3.24 & 3.84 & 5.54 & 7.12 & 7.99 & 4.59 & 4.70 & 4.88 & 5.05 & 5.19 \\
WASP-133 b & 1.27 & 3.19 & 4.11 & 5.49 & 6.81 & 8.04 & 4.59 & 4.70 & 4.88 & 5.05 & 5.19 \\
TOI-172 b & 1.40 & 3.08 & 3.31 & 3.90 & 5.30 & 10.60 & 4.59 & 4.77 & 4.91 & 5.00 & 5.09 \\
TOI-1296 b & 1.40 & 3.16 & 3.66 & 4.77 & 5.80 & 6.76 & 4.59 & 4.77 & 4.91 & 5.00 & 5.09 \\
TrES-3 b & 1.40 & 3.26 & 4.22 & 5.21 & 6.73 & 7.45 & 4.59 & 4.77 & 4.91 & 5.00 & 5.09 \\
HAT-P-59 b & 1.56 & 3.12 & 3.68 & 4.72 & 5.79 & 10.59 & 4.55 & 4.70 & 4.86 & 4.98 & 5.06 \\
HAT-P-62 b & 1.56 & 3.18 & 3.96 & 5.28 & 6.48 & 8.83 & 4.55 & 4.70 & 4.86 & 4.98 & 5.06 \\
HATS-8 b & 1.56 & 3.25 & 4.18 & 5.51 & 6.76 & 8.01 & 4.55 & 4.70 & 4.86 & 4.98 & 5.06 \\
WASP-4 b & 1.56 & 3.30 & 4.00 & 5.74 & 7.14 & 7.84 & 4.55 & 4.70 & 4.86 & 4.98 & 5.06 \\
WASP-19 b & 1.56 & 3.27 & 3.99 & 5.64 & 7.22 & 8.10 & 4.55 & 4.70 & 4.86 & 4.98 & 5.06 \\
HATS-34 b & 1.73 & 3.22 & 4.10 & 5.64 & 6.99 & 7.58 & 4.48 & 4.66 & 4.81 & 4.92 & 5.00 \\
HATS-44 b & 1.73 & 3.30 & 4.09 & 5.38 & 6.68 & 7.41 & 4.48 & 4.66 & 4.81 & 4.92 & 5.00 \\
HATS-76 b & 1.73 & 3.25 & 4.06 & 5.25 & 6.33 & 6.93 & 4.48 & 4.66 & 4.81 & 4.92 & 5.00 \\
WASP-50 b & 1.73 & 3.15 & 3.80 & 5.10 & 6.37 & 7.17 & 4.48 & 4.66 & 4.81 & 4.92 & 5.00 \\
HAT-P-19 b & 1.92 & 3.19 & 3.96 & 5.35 & 6.41 & 7.10 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HAT-P-20 b & 1.92 & 3.13 & 3.67 & 4.77 & 5.84 & 9.71 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HAT-P-37 b & 1.92 & 3.11 & 3.67 & 4.85 & 6.07 & 6.85 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HAT-P-53 b & 1.92 & 3.16 & 4.04 & 5.55 & 6.73 & 7.44 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HATS-32 b & 1.92 & 3.15 & 3.75 & 5.11 & 6.34 & 7.00 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HATS-33 b & 1.92 & 3.14 & 3.80 & 5.03 & 6.10 & 6.84 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
HATS-43 b & 1.92 & 3.14 & 3.84 & 5.21 & 6.42 & 7.25 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
Kepler-412 b & 1.92 & 3.19 & 3.91 & 5.26 & 6.62 & 7.47 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
Kepler-426 b & 1.92 & 3.12 & 3.70 & 5.39 & 6.57 & 7.40 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
TOI-3757 b & 1.92 & 3.25 & 3.93 & 5.31 & 6.65 & 7.28 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
Kepler-428 b & 1.92 & 3.11 & 3.64 & 4.74 & 5.89 & 6.71 & 4.51 & 4.67 & 4.83 & 4.92 & 4.98 \\
CoRoT-12 b & 2.12 & 3.17 & 4.10 & 5.58 & 6.75 & 7.57 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
HAT-P-52 b & 2.12 & 3.09 & 3.78 & 4.96 & 6.06 & 6.71 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
HAT-P-55 b & 2.12 & 3.15 & 3.80 & 5.02 & 6.11 & 7.03 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
HATS-5 b & 2.12 & 3.11 & 3.55 & 4.40 & 5.34 & 6.38 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
HATS-14 b & 2.12 & 3.18 & 3.77 & 4.86 & 5.98 & 6.80 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
HATS-57 b & 2.12 & 3.15 & 3.73 & 4.69 & 5.61 & 6.21 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
Kepler-425 b & 2.12 & 3.20 & 3.93 & 5.56 & 6.68 & 7.47 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
WASP-5 b & 2.12 & 3.21 & 4.00 & 5.28 & 6.53 & 7.50 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
WASP-6 b & 2.12 & 3.21 & 4.03 & 5.79 & 6.88 & 7.56 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
WASP-22 b & 2.12 & 3.10 & 3.51 & 4.51 & 5.56 & 6.35 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
WASP-23 b & 2.12 & 3.15 & 3.71 & 4.86 & 5.96 & 6.70 & 4.40 & 4.61 & 4.75 & 4.87 & 4.98 \\
CoRoT-5 b & 2.35 & 3.33 & 4.20 & 5.22 & 6.75 & 7.41 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
HAT-P-25 b & 2.35 & 3.20 & 4.00 & 5.06 & 6.01 & 6.77 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
HAT-P-54 b & 2.35 & 3.12 & 3.55 & 4.57 & 5.59 & 6.36 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
HATS-11 b & 2.35 & 3.19 & 4.04 & 5.29 & 6.35 & 7.03 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
HATS-28 b & 2.35 & 3.17 & 3.86 & 5.19 & 6.42 & 7.21 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
WASP-89 b & 2.35 & 4.44 & 4.83 & 5.31 & 6.08 & 8.20 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
WASP-119 b & 2.35 & 3.24 & 4.01 & 5.31 & 6.57 & 7.31 & 4.44 & 4.56 & 4.73 & 4.88 & 4.97 \\
CoRoT-29 b & 2.61 & 3.16 & 3.86 & 5.13 & 6.31 & 9.36 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HAT-P-28 b & 2.61 & 3.13 & 3.62 & 5.03 & 6.28 & 6.98 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HAT-P-51 b & 2.61 & 3.27 & 4.06 & 5.47 & 6.51 & 7.35 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HAT-P-61 b & 2.61 & 3.12 & 3.97 & 5.13 & 6.37 & 8.66 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HAT-P-63 b & 2.61 & 3.14 & 3.73 & 5.01 & 6.15 & 6.78 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HATS-13 b & 2.61 & 3.13 & 3.75 & 5.09 & 6.19 & 7.05 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HATS-23 b & 2.61 & 3.16 & 3.70 & 5.43 & 6.85 & 7.49 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
HATS-25 b & 2.61 & 3.14 & 3.86 & 4.89 & 6.34 & 7.03 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
K2-30 b & 2.61 & 3.12 & 3.65 & 4.65 & 5.48 & 6.13 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
K2-132 b & 2.61 & 3.04 & 3.21 & 3.57 & 3.93 & 4.41 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
K2-140 b & 2.61 & 3.14 & 3.78 & 4.73 & 5.63 & 6.44 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
Kepler-44 b & 2.61 & 3.10 & 3.53 & 4.77 & 5.67 & 6.62 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
TOI-905 b & 2.61 & 3.17 & 3.67 & 4.60 & 5.83 & 6.67 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
TOI-3629 b & 2.61 & 3.13 & 3.64 & 4.61 & 5.65 & 6.68 & 4.52 & 4.62 & 4.71 & 4.79 & 4.87 \\
CoRoT-16 b & 2.89 & 3.23 & 4.10 & 6.03 & 7.01 & 7.89 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
CoRoT-23 b & 2.89 & 5.04 & 5.41 & 6.33 & 9.37 & 11.52 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
WASP-59 b & 2.89 & 3.04 & 3.25 & 3.68 & 4.32 & 4.86 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
WASP-124 b & 2.89 & 3.10 & 3.67 & 4.65 & 5.68 & 6.30 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
WASP-185 b & 2.89 & 4.03 & 4.50 & 5.02 & 5.62 & 6.25 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
HAT-P-58 b & 2.89 & 3.18 & 3.93 & 5.06 & 6.14 & 6.96 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
HATS-29 b & 2.89 & 3.14 & 3.87 & 4.88 & 6.02 & 6.80 & 4.46 & 4.55 & 4.64 & 4.74 & 4.83 \\
HATS-47 b & 3.21 & 3.15 & 3.93 & 5.19 & 6.27 & 6.95 & 4.38 & 4.49 & 4.56 & 4.65 & 4.74 \\
TOI-2158 b & 3.21 & 3.05 & 3.24 & 4.01 & 4.82 & 5.39 & 4.38 & 4.49 & 4.56 & 4.65 & 4.74 \\
Kepler-12 b & 3.56 & 3.17 & 3.81 & 4.82 & 5.84 & 6.42 & 4.32 & 4.50 & 4.58 & 4.66 & 4.74 \\
TOI-2669 b & 3.56 & 3.13 & 3.86 & 5.02 & 6.15 & 6.91 & 4.32 & 4.50 & 4.58 & 4.66 & 4.74 \\
WASP-151 b & 3.56 & 3.17 & 3.62 & 4.82 & 5.69 & 6.34 & 4.32 & 4.50 & 4.58 & 4.66 & 4.74 \\
TOI-1268 b & 3.95 & 3.03 & 3.24 & 3.63 & 4.00 & 4.52 & 4.26 & 4.51 & 4.61 & 4.71 & 4.85 \\
CoRoT-30 b & 4.38 & 3.02 & 3.14 & 3.49 & 4.62 & 5.22 & 4.26 & 4.50 & 4.62 & 4.78 & 4.92 \\
TOI-559 b & 6.62 & 3.62 & 3.98 & 4.84 & 6.03 & 7.83 & 4.43 & 4.61 & 4.88 & 5.13 & 5.34 \\
\end{tabular}

